AR as an Evaluation Playground: Bridging Metrics and Visual Perception of Computer Vision Models

Quantitative metrics are central to evaluating computer vision (CV) models, but they often fail to capture real-world performance due to protocol inconsistencies and ground-truth noise. While visual perception studies can complement these metrics, they often require end-to-end systems that are time-consuming to implement and setups that are difficult to reproduce. We systematically summarize key challenges in evaluating CV models and present the design of ARCADE, an evaluation platform that leverages augmented reality (AR) to enable easy, reproducible, and human-centered CV evaluation. ARCADE uses a modular architecture that provides cross-platform data collection, pluggable model inference, and interactive AR tasks, supporting both metric and visual perception evaluation. We demonstrate ARCADE through a user study with 15 participants and case studies on two representative CV tasks, depth and lighting estimation, showing that ARCADE can reveal perceptual flaws in model quality that are often missed by traditional metrics. We also evaluate ARCADE's usability and performance, showing its flexibility as a reliable real-time platform.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016
modified by Matt Brehmer, Feb 2024

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE VIS: Visualization & Visual Analytics (Short Papers, Posters)
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> sections/EvalCase.tex <==
\section{Performance Evaluation \& Case Studies}\label{sec:implementation_evaluation}


\begin{table}[t]
\centering
\caption{
Frame rate (FPS) for live streaming and replay streams at different resolutions over campus Wi-Fi. Live streaming reflects real-time transmission from the AR device to the browser, while replay denotes the performance when rendering recorded sequences.
}
\label{tab:fps_network}
\small
\begin{tabular}{l|c|c}
\toprule
\textbf{Resolution} & \textbf{Live Streaming (FPS)} & \textbf{Replay (FPS)} \\
\midrule
640 $\times$ 480 (SD)     & 22 & 30 \\
1280 $\times$ 720 (HD)    & 14 & 27 \\
1920 $\times$ 1080 (FHD)  & 10 & 22 \\
\bottomrule
\end{tabular}
\vspace{-0.4cm}
\end{table}


\begin{table}[t]
\centering
\caption{
Interaction latency (in milliseconds) across different resolutions for three key components: RC car control, point cloud streaming, and plane interaction. Latency values are measured over an institute campus Wi-Fi network and represent the end-to-end responsiveness of each interaction type. RC Car Latency for sending and executing commands is 38 ms.
}
\label{tab:interaction_latency}
\small
\begin{tabular}{l|c|c}
\toprule
\textbf{Resolution}  & \textbf{Point Cloud (ms)} & \textbf{Obj Interaction (ms)} \\
\midrule
640 $\times$ 480 (SD)     & 19 $\pm$ 3.2  & 7.52 $\pm$ 2.5 \\
1280 $\times$ 720 (HD)    & 33.5 $\pm$ 7.3  & 12.3 $\pm$ 10.5 \\
1920 $\times$ 1080 (FHD)  & 57.1 $\pm$ 9  & 10.2 $\pm$ 5.6 \\
\bottomrule
\end{tabular}
\vspace{-0.5cm}
\end{table}

\subsection{System Evaluation}
\label{Evaluation}

We evaluate \sysname using a unified setup where captures are collected on an iPhone~14 Pro and streamed to an edge server equipped with an NVIDIA RTX~4090 GPU, a 13th~Gen Intel i9-13900K CPU, and 128\,GB of RAM. All inference is executed on the server, and both benchmark metrics and visual outputs are recorded for replay. Our evaluation tries to capture different aspects of \sysname on two fronts: (i) computational overhead of the rendering pipeline and (ii) end-to-end latency over wireless networks, with results summarized in Tables~\ref{tab:component_perf}, \ref{tab:fps_network}, and~\ref{tab:interaction_latency}. Experiments are conducted on campus Wi-Fi where the AR device, edge server, and web client share the same access point. The render–composite loop runs in real-time across all tested resolutions—5.2\,ms at $640{\times}480$ and 23\,ms at $1920{\times}1080$—allowing replay above 20\,FPS. Running DepthAnything~V2-Base adds 45–74\,ms per frame, but replay remains at 23\,FPS at SD resolution. In live streaming mode, we achieve 22\,FPS at $640{\times}480$; higher resolutions are feasible but introduce additional latency. In the following subsections we will show evaluation results for different features and components of \sysname.

\subsubsection{Cross-Renderer Geometry Correctness.}
To ensure that evaluations carried out on our server truly reflect what would happen on-device, we verify that server-side rendering faithfully reproduces ARKit geometry. We use the phone as the reference renderer by snapshotting the virtual layer in an \emph{ARKit-parity} mode (solid-black background, unlit white material, shadows off), and render the same object(s) on the server with matched intrinsics and poses in an equivalent mode (unlit, no shadows, $2\times$ supersampling). We then compare binary masks from both sides using Silhouette IoU, Boundary F-score (2\,px tolerance), and scale error, isolating geometry and alpha from photometric effects. Results show perfect pixel-level agreement: Silhouette IoU and Boundary F1 both reach $1.0 \pm 0.0$, and the scale error is $0.0 \pm 0.0$\%. These results confirm that researchers can treat the server’s rendering as geometrically identical to ARKit, gaining the same fidelity as on-device evaluation but in a simpler, scriptable, and more scalable framework.



\subsubsection{Micro-benchmark}
Table~\ref{tab:component_perf} details the per-component latencies of our system across three different resolutions. Due to the optimizations and implementation choices that we discussed in \S\ref{subsec:implementation}. Our current configuration achieves real-time performance. Notably, based on the optimizations that we have for streaming and client-side compression, our optimized rendering and compositing pipeline reduces latency significantly from an initial baseline of approximately 300\,ms per frame to just 5.2\,ms at 640$\times$480 resolution. These results underscore the effectiveness of our architectural and algorithmic enhancements, ensuring responsive and scalable AR experiences.


\subsubsection{Interaction}
Table~\ref{tab:interaction_latency} reports end‑to‑end latencies for two interactive features—object/plane manipulation and RC‑car control. We observe that object and plane updates are highly responsive. The object interaction latency ranges from 7.5~ms at SD to 12~ms at FHD, so adjustments appear almost instantaneously. RC‑car commands average 38~ms round‑trip over the same Wi‑Fi network, and execution on the vehicle side adds only about 1~ms.


\subsubsection{Replay and Live Stream}
Table~\ref{tab:fps_network} shows the frame rates achieved in both live‑streaming and replay modes. Replay meets real‑time requirements at every resolution because frames are rendered on the server from pre‑recorded data, avoiding network upload and on‑device delays. Live streaming reaches 22~FPS at $640\times480$, which satisfies the frame‑rate target for most mobile AR applications. Without doing optimization for rendering we got FPS of 3 for live stream.  For point cloud streaming, we transmit data in the \texttt{.pcd} format, which is roughly 75\% smaller than \texttt{.ply} (around 1.8Mb). Combined with Open3D’s built‑in compression, this keeps point‑cloud latency below 60~ms even at 1080p. Since this feature doesn't need real-time interactions, this latency should be sufficient for smooth 3D scene analysis.


\subsection{Dataset}
\label{subsec:casestudy_dataset}

To support our case studies, we built a small evaluation dataset. 
All sequences were recorded with an iPhone~14 Pro, streamed to the edge server, and saved for replay across different tasks and models. 
The dataset includes a 407-frame video, designed to highlight challenges such as reflective surfaces, large occlusion boundaries, and complex indoor lighting. Although the dataset is not large, it serves as a controlled benchmark for \sysname: each capture can be reused across multiple evaluation pipelines, enabling fair comparisons and reproducible case studies.


\subsection{Case Studies: Depth and Lighting}
\label{sec:caseStudy}

Depth estimation and lighting estimation are long-standing computer vision problems, each with established datasets and benchmark metrics. Depth models are typically judged by RMSE or $\delta$ thresholds, while lighting models are evaluated with angular error or RMSE on environment maps. Although these metrics enable large-scale benchmarking, they often fail to capture how models behave in realistic visual contexts. Small numerical differences can correspond to large perceptual artifacts, and in some cases different metrics even lead to contradictory rankings. 

To highlight these limitations, we conduct two case studies using \sysname. Depth estimation serves as an example of a geometry-centric CV task, while lighting estimation represents an appearance-centric task. Together they illustrate two points: first, the usefulness of \sysname in exposing evaluation blind spots through perceptual visualization; and second, the findings that such analysis reveals about state-of-the-art CV models.


\subsubsection{Depth Estimation}


\begin{table}[t]
\centering
\caption{Performance comparison on the NYU Depth V2~\cite{Silberman:ECCV12}}
\label{tab:performance_nyu_SIDE}
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}l|lrrrrr@{}}
\toprule
\textbf{Model}  & \textbf{RMSE} $\downarrow$ & \textbf{AbsRel} $\downarrow$ & \textbf{$\delta_1$} $\uparrow$ & \textbf{$\delta_2$} $\uparrow$ & \textbf{$\delta_3$} $\uparrow$ \\
\midrule
DPT~\cite{Ranftl2021}  & 0.357 & 0.104 & 0.904 & 0.988 & 0.998 \\
ZoeDepth~\cite{https://doi.org/10.48550/arxiv.2302.12288}\tnote{$\dagger$}  & 0.270 & 0.075 & 0.960 & 0.995 & 0.999 \\
ECoDepth~\cite{Patni_2024_CVPR}  & 0.218 & 0.059 & 0.970 & 0.997 & 0.999 \\
Depth AnythingV1~\cite{depth_anything_v1} & {0.206} & {0.056} & {0.980} & {0.998} & {0.999} \\
Depth AnythingV2~\cite{depth_anything_v2} & \textbf{{0.206}} & \textbf{{0.056}} & \textbf{{0.984}} & \textbf{{0.998}} &\textbf{ {1.000}} \\

\bottomrule
\end{tabular}
}
\vspace{-0.5cm}
\end{table}


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{assets/depth_cs_pointcloud.pdf}
    \caption{Viewing teapot placement from different angels by using \sysname's point cloud features. 
    % First row shows the 2D object placement, third row show the point cloud view.
    }
    \label{fig:depth_cs_pointcloud}
    \vspace{-0.5cm}
\end{figure}



\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{assets/Depth_CS_screenshot.pdf}
    \caption{
    % A screenshot of \sysname's UI that displays quantitative metrics alongside the depth and object placement visualizations for a captured scene.
    Screenshot of \sysname's UI showing metrics alongside depth and object placement visualizations for a captured scene.
    }
    \label{fig:depth_casestudy_screenshot}
    % \vspace{-0.5cm}
\end{figure}



\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{assets/depth_cs_plane1.pdf}
        \caption{Plane set to 0.75m for ARKit, and 1.3m for DepthAnything V2 and ZoeDepth. Visualization highlights depth estimation differences across methods.}
        \label{fig:depth_cs_dynamic_plane}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{assets/depth_cs_plane2.pdf}
        \caption{Plane set to 0.95m. Different frames of the same scene are shown to evaluate spatial detail and temporal smoothness.
        }
        \label{fig:depth_cs_fixed_plane}
    \end{subfigure}
    \caption{Depth visualization case study at different plane distances and across different frames of the same scene. Red represents closer depth values, while blue indicates farther distances.}
    \label{fig:depth_casestudy_plane}
    % \vspace{-0.5cm}
\end{figure*}


we did the Depth case study through three representative depth pipelines---Depth Anything V2 (metric depth version)~\cite{depth_anything_v2}, ZoeDepth~\cite{https://doi.org/10.48550/arxiv.2302.12288}, and the ARKit~\cite{AppleARkit}. 
Below we list three findings with the use of \sysname.


\para{Occlusion Consistency and Plane Rendering.} Our framework enables both raw depth-map visualizations and interactive plane placements to evaluate occlusion consistency across different models. In Figure~\ref{fig:depth_casestudy_plane}, we place virtual planes in each scene to assess how accurately and consistently each model predicts depth.

First, we observe significant variation in global scale across methods. In Figure~\ref{fig:depth_cs_dynamic_plane}, the virtual plane needs to be positioned at 0.75m when using ARKit depth. However, to achieve an equivalent occlusion with DepthAnythingV2 and ZoeDepth, the plane must be placed nearly twice as far—at 1.3 m. This reveals a consistent overestimation of metric depth by these models, which can severely impact spatial coherence in AR scenes. In Figure~\ref{fig:depth_cs_fixed_plane}, we fix the plane at 0.95~m across all methods. Ideally, the occlusion should appear similar in each view, but significant discrepancies remain, highlighting issues with depth scale consistency.

Second, the quality of local boundaries varies notably. For example, ARKit struggles with reflective surfaces like a laptop monitor—shown in the blue boxes(Figure~\ref{fig:depth_cs_fixed_plane})—causing the occlusion plane to appear incorrectly over the monitor. Similarly, ZoeDepth completely fails to capture the structure of the large monitor, as highlighted by the red box in Figure~\ref{fig:depth_cs_fixed_plane}. While these artifacts may be subtle in the color-coded depth maps, they become starkly visible in the rendered occlusion views, emphasizing the value of task-driven visualizations.


\para{Temporal Consistency.}
We evaluate \emph{temporal consistency} using the replay feature of our system (\S\ref{subsec:ARTask}). This experiment reveals that all models, including ARKit~\cite{AppleARkit}, struggle to maintain stable object and plane placements over time, highlighting a common limitation in temporal consistency. Among these models, our replay analysis shows that DepthAnythingV2 performed best in terms of visual stability.

To quantify \emph{temporal consistency}, we use the \emph{Optical flow-based OPW} metric, following NVDS~\cite{NVDS}. OPW measures temporal stability by computing the frame-to-frame warping error between rendered depth predictions using estimated optical flow. It is formally defined as:

\begin{equation}
\text{OPW} = \frac{1}{N - 1} \sum_{n=2}^{N} \mathcal{L}^t(n, n-1),
\end{equation}

where $\mathcal{L}^t(n, n-1)$ denotes the temporal warping loss between consecutive frames $n$ and $n-1$, and $N$ is the total number of frames. Lower OPW values indicate smoother and more consistent depth predictions across time. Our evaluation shows that DepthAnythingV2 achieves the best temporal consistency with an OPW of 0.019. ARKit follows with an OPW of 0.032, while ZoeDepth exhibits the highest temporal inconsistency with an OPW of 0.052. These results are aligned with our visual observations.

%  ----------------------------------------------------------------------------------


% fig:experiment_protocols
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{assets/experiment_protocols.pdf}
    \caption{Lighting estimation experiment protocol overview. \textnormal{We evaluate the accuracy of lighting estimation models by directly comparing the estimated environment maps (left) and three rendered virtual spheres of different materials (right).}}
\label{fig:experiment_protocols}
\vspace{-0.3cm}
\end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% fig:case_study_lighting_result_visualizations
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{assets/lighting_estimation_case_study.pdf}
    \caption{Lighting estimation rendering visualizations. \textnormal{The \sysname visualization interface enables side-by-side display of virtual teapots under varying rendering parameters, such as different materials and lighting conditions. This design facilitates perceptual-based evaluation studies by supporting frame-by-frame visualization of numerical results from Table~\ref{tab:eval_three_sphere_reorganized}}.
    }
\label{fig:case_study_lighting_result_visualizations}
% \vspace{-0.5cm}
\end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsubsection{Lighting Estimation}



We evaluate three representative lighting estimation models: XiheNet~\cite{xihe_mobisys2021}, StyleLight~\cite{wang2022stylelight}, and DiffusionLight~\cite{Phongthawee2023DiffusionLight}, covering lightweight, mid-sized, and large-scale designs. XiheNet runs efficiently but produces only low-frequency environment maps; StyleLight improves visual quality; DiffusionLight achieves the highest fidelity at greater computational cost. All models run in \sysname as containerized programs.

For numerical evaluation, we use the Laval Indoor HDR dataset~\cite{Gardner2017} and report angular error, Si-RMSE, and RMSE. We also implement the \emph{three-sphere protocol}~\cite{wang2022stylelight}, which compares renderings of diffuse, matte, and mirror spheres under estimated lighting (Fig.~\ref{fig:experiment_protocols}). While such protocols are normally complex to set up, \sysname provides them as built-in, reproducible options. For perceptual evaluation we used \sysname and plugged the inference model into the system as a containerized docker files and used our AR-Tasks~\S~\ref{subsec:ARTask} to get the final renderings.



\para{Object Appearance and Spatial Context.} 
As we discussed in the \S~\ref{sec:perceptionGap}, our experiments reveals that different numerical metrics often highlight different aspects of lighting estimation performance. To better understand these numerical discrepancies, we use \sysname to visualize each model’s predictions under the same input conditions. As shown in Figure~\ref{fig:case_study_lighting_result_visualizations}, relit teapot rendered using different models reveal perceptual differences not captured in the numerical scores. While the quantitative metrics suggest that DiffusionLight performs best, visual inspection of the rendered objects uncovers nuanced issues, such as unnatural brightness or missing directional shadows. These issues would otherwise remain hidden in numerical-only evaluation. Thus, it is important to supplement numerical results with perceptual analysis when evaluating lighting estimation for AR.

We also observed that small inaccuracies in estimated light directions or intensities lead to large differences in object appearance, particularly in materials with specular components. For example, relighting with XiheNet resulted in over-smoothing of specular highlights, making the metallic teapot appear dull. By contrast, DiffusionLight sometimes overestimated intensity, causing teapots to look unnaturally bright under realistic indoor conditions. These artifacts are difficult to assess from environment maps alone, but become obvious when rendered into the AR scene using \sysname.



\subsubsection{Discussion and Implications}

Our case studies on depth and lighting estimation highlight the central message of this paper: benchmark numbers alone do not guarantee perceptual quality in AR applications. DepthAnything V2 and ZoeDepth, despite strong performance on NYU Depth V2, still over-estimate scale, jitter over time, and blur object boundaries, leading to visible artifacts in placement and occlusion tasks. Lighting models such as XiheNet, StyleLight, and DiffusionLight show a similar gap--two models with comparable angular error or RMSE can produce noticeably different renderings, especially on reflective or complex materials. By reusing the same captured scenes across all model–metric–task combinations, \sysname enabled us to diagnose these issues under identical conditions, combining metrics with direct AR visualizations such as point clouds, occlusion renders, and relit objects. This capture-once-evaluate-many workflow revealed temporal instabilities, scale errors, and lighting artifacts that benchmarks alone obscure, demonstrating how application-grounded evaluation with \sysname complements traditional metrics and leads to a more complete understanding of CV model behavior.


==> sections/caseStudyDepth.tex <==
\section{Case Study: Depth}




\begin{table}[t]
\centering
\caption{Performance comparison on the NYU Depth V2~\cite{Silberman:ECCV12}}
\label{tab:performance_nyu_SIDE}
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}l|lrrrrr@{}}
\toprule
\textbf{Model}  & \textbf{RMSE} $\downarrow$ & \textbf{AbsRel} $\downarrow$ & \textbf{$\delta_1$} $\uparrow$ & \textbf{$\delta_2$} $\uparrow$ & \textbf{$\delta_3$} $\uparrow$ \\
\midrule
DPT~\cite{Ranftl2021}  & 0.357 & 0.104 & 0.904 & 0.988 & 0.998 \\
ZoeDepth~\cite{https://doi.org/10.48550/arxiv.2302.12288}\tnote{$\dagger$}  & 0.270 & 0.075 & 0.960 & 0.995 & 0.999 \\
ECoDepth~\cite{Patni_2024_CVPR}  & 0.218 & 0.059 & 0.970 & 0.997 & 0.999 \\
Depth AnythingV1~\cite{depth_anything_v1} & {0.206} & {0.056} & {0.980} & {0.998} & {0.999} \\
Depth AnythingV2~\cite{depth_anything_v2} & \textbf{{0.206}} & \textbf{{0.056}} & \textbf{{0.984}} & \textbf{{0.998}} &\textbf{ {1.000}} \\

\bottomrule
\end{tabular}
}
\vspace{-0.5cm}
\end{table}


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{assets/depth_cs_pointcloud.pdf}
    \caption{Viewing teapot placement from different angels by using \sysname's point cloud features. 
    % First row shows the 2D object placement, third row show the point cloud view.
    }
    \label{fig:depth_cs_pointcloud}
    \vspace{-0.5cm}
\end{figure}



\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{assets/Depth_CS_screenshot.pdf}
    \caption{
    % A screenshot of \sysname's UI that displays quantitative metrics alongside the depth and object placement visualizations for a captured scene.
    Screenshot of \sysname's UI showing metrics alongside depth and object placement visualizations for a captured scene.
    }
    \label{fig:depth_casestudy_screenshot}
    \vspace{-0.5cm}
\end{figure}



\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{assets/depth_cs_plane1.pdf}
        \caption{Plane set to 0.75m for ARKit, and 1.3m for DepthAnything V2 and ZoeDepth. Visualization highlights depth estimation differences across methods.}
        \label{fig:depth_cs_dynamic_plane}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{assets/depth_cs_plane2.pdf}
        \caption{Plane set to 0.95m. Different frames of the same scene are shown to evaluate spatial detail and temporal smoothness.
        }
        \label{fig:depth_cs_fixed_plane}
    \end{subfigure}
    \caption{Depth visualization case study at different plane distances and across different frames of the same scene. Red represents closer depth values, while blue indicates farther distances.}
    \label{fig:depth_casestudy_plane}
    \vspace{-0.5cm}
\end{figure*}




\label{sec:casestudy:depth}

Depth is a fundamental part of AR realism: every virtual-real interaction---object placement, occlusion, scene relighting---depends on accurate, \emph{perceptually plausible} depth.  Yet, as noted in \S\ref{sec:introduction}, benchmark metrics such as RMSE and $\delta$ scores often disagree and say little about how a model behaves once rendered in context, and they often fail to capture the complexities of the real-world deployment systems. In this case study, we demonstrate how we can use\sysname to uncover common evaluation pitfalls. 


\subsection{\sysname Setup}

We record a 407-frames video by using \sysname client and replay it through three representative depth pipelines---Depth Anything V2 (metric depth version)~\cite{depth_anything_v2}, ZoeDepth~\cite{https://doi.org/10.48550/arxiv.2302.12288}, and the ARKit~\cite{AppleARkit}. The same capture is then routed into three perception-oriented AR tasks, i.e., occlusion-plane rendering, object rendering, and 3D point-cloud inspection, while conventional depth metrics are logged frame by frame. The key evaluation question is to understand if and how qualitative metric performance translates to perceptually correct object placement, consistent occlusions, and stable temporal behavior in a realistic AR scene.


The edge server runs on a machine with an NVIDIA RTX~4090 GPU, a 13th~Gen Intel i9-13900K CPU, and 128\,GB of RAM. All data is captured on an iPhone~14~Pro, which streams sensor information and metadata to the server in real time. All model inference tasks are performed on the edge server, and the results, along with the original sensor data, are saved for side-by-side comparison via our replay interface in addition to captured physical scenes. 
% In this case study, the video consisting of 407 frames shown in Figure~\ref{fig:depth_cs_pointcloud} was captured once using our data collection tool and replayed multiple times with different configurations for comparison and analysis.

\subsection{Interesting Findings}
Below we list three findings with the use of \sysname.



\para{Occlusion Consistency and Plane Rendering.} Our framework enables both raw depth-map visualizations and interactive plane placements to evaluate occlusion consistency across different models. In Fig.~\ref{fig:depth_casestudy_plane}, we place virtual planes in each scene to assess how accurately and consistently each model predicts depth.

First, we observe significant variation in global scale across methods. In Fig.~\ref{fig:depth_cs_dynamic_plane}, the virtual plane needs to be positioned at 0.75m when using ARKit depth. However, to achieve an equivalent occlusion with DepthAnythingV2 and ZoeDepth, the plane must be placed nearly twice as far—at 1.3m. This reveals a consistent overestimation of metric depth by these models, which can severely impact spatial coherence in AR scenes. In Fig.~\ref{fig:depth_cs_fixed_plane}, we fix the plane at 0.95~m across all methods. Ideally, the occlusion should appear similar in each view, but significant discrepancies remain, highlighting issues with depth scale consistency.

Second, the quality of local boundaries varies notably. For example, ARKit struggles with reflective surfaces like a laptop monitor—shown in the blue boxes(Fig.~\ref{fig:depth_cs_fixed_plane})—causing the occlusion plane to appear incorrectly over the monitor. Similarly, ZoeDepth completely fails to capture the structure of the large monitor, as highlighted by the red box in Fig.~\ref{fig:depth_cs_fixed_plane}. While these artifacts may be subtle in the color-coded depth maps, they become starkly visible in the rendered occlusion views, emphasizing the value of task-driven visualizations.


\para{Temporal Consistency.}
We evaluate \emph{temporal consistency} using the replay feature of our system (\S\ref{subsec:ARTask}). This experiment reveals that all models, including ARKit~\cite{AppleARkit}, struggle to maintain stable object and plane placements over time, highlighting a common limitation in temporal consistency. Among these models, our replay analysis shows that DepthAnythingV2 performed best in terms of visual stability.

To quantify \emph{temporal consistency}, we use the \emph{Optical flow-based OPW} metric, following NVDS~\cite{NVDS}. OPW measures temporal stability by computing the frame-to-frame warping error between rendered depth predictions using estimated optical flow. It is formally defined as:

\begin{equation}
\text{OPW} = \frac{1}{N - 1} \sum_{n=2}^{N} \mathcal{L}^t(n, n-1),
\end{equation}

where $\mathcal{L}^t(n, n-1)$ denotes the temporal warping loss between consecutive frames $n$ and $n-1$, and $N$ is the total number of frames. Lower OPW values indicate smoother and more consistent depth predictions across time. Our evaluation shows that DepthAnythingV2 achieves the best temporal consistency with an OPW of 0.019. ARKit follows with an OPW of 0.032, while ZoeDepth exhibits the highest temporal inconsistency with an OPW of 0.052. These results are aligned with our visual observations.



\begin{tcolorbox}[colback=gray!10, colframe=gray!50!black, boxrule=0.5pt, arc=2pt, left=4pt, right=4pt, top=2pt, bottom=2pt]
\textbf{Key Takeaway.} \sysname can expose different types of errors and visual artifacts, offering a richer perspective than numerical evaluation alone in understanding CV model performance.
The qualitative artifacts highlighted here suggest the need for metrics, e.g. scale-aware RMSE or temporal OPW thresholds, that better align with perceptual quality. 
\end{tcolorbox}



\subsection{Discussion and Implications}

The depth case study reinforces the central message of this paper: \emph{benchmark numbers alone do not guarantee perceptual quality in real applications such as AR}.  DepthAnything V2 and ZoeDepth rank highly on NYU Depth V2, yet both over-estimate scale and jitter over time, producing clearly visible artifacts in object placement and occlusion tasks.

Beyond these specific findings, our results underscore a broader need for application-centric evaluation methodologies. By providing an interactive environment, \sysname reveals failure modes that might remain hidden in traditional quantitative evaluations. For instance, viewing point clouds from multiple angles exposes the depth miss estimations, and replaying recorded sequences highlights temporal instability across frames. These deeper insights can guide future model refinements, particularly for use cases demanding continuous AR interaction.


By reusing a single capture across all model-metric-task combinations, \sysname lets researchers debug depth scale, boundary detail, and temporal smoothness under identical conditions. 
This \emph{capture-once-evaluate-many} workflow streamlines ablation studies and enables fairer comparisons across the community.



==> sections/casesStudyLighting.tex <==
\section{Case Study 2: Lighting Estimation}
\label{sec:casestudy:lighting}

In this section, we conduct another case study to demonstrate how \sysname enables perceptually grounded evaluation of lighting models, by 
\1 Supporting numerical evaluations under standardized protocols such as the Laval dataset~\cite{Gardner2017} and three-sphere benchmark~\cite{wang2022stylelight}; \2 allowing users to visualize estimated environment maps and applied lighting effects directly on rendered virtual objects. 
We choose to evaluate this type of model because it is a fundamental CV task and is also widely used in AR applications to achieve visually coherent and realistic rendering~\cite{xihe_mobisys2021,wang2022stylelight,Gardner2017,somanath-envmapnet}. 
Unlike depth estimation that aims to produce metric-accurate and sharp details on estimation results, the key interest of lighting estimation often lies in reliably extrapolating physical environment observations to create lighting representations, e.g., environment map. Similar to depth estimation evaluations, conventional metrics (e.g., angular error, RMSE) often fail to reflect the estimation quality, particularly in human-perceived visual qualities. 

% fig:experiment_protocols
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{assets/experiment_protocols.pdf}
    \caption{Lighting estimation experiment protocol overview. We evaluate the accuracy of lighting estimation models by directly comparing the estimated environment maps (left) and three rendered virtual spheres of different materials (right).}
\label{fig:experiment_protocols}
\vspace{-0.3cm}
\end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% tab:eval_three_sphere_reorganized
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\centering
\caption{
Quantitative evaluation of environment maps and the three-sphere protocol. We test three representative lighting estimation models: XiheNet~\cite{xihe_mobisys2021}, StyleLight~\cite{wang2022stylelight}, and DiffusionLight~\cite{Phongthawee2023DiffusionLight} under the standard test setting with a single 75$^\circ$ horizontal FoV input. We noticed major misalignment on different evaluation metrics. Specifically, models that perform well on RMSE and Si-RMSE may not yield good angular error numbers.
}
\label{tab:eval_three_sphere_reorganized}
\resizebox{\columnwidth}{!}{
\begin{tabular}{llccc}
\toprule
\textbf{Target} & \textbf{Model} & \textbf{Angular Error $\downarrow$} & \textbf{Si-RMSE $\downarrow$} & \textbf{RMSE $\downarrow$} \\
\midrule
\multirow{3}{*}{\shortstack[l]{Env.\\Map}} 
    & XiheNet~\cite{xihe_mobisys2021} & 7.39 & 0.23 & 0.34 \\
    & StyleLight~\cite{wang2022stylelight} & 5.81 & 0.27 & 0.25 \\
    & DiffusionLight~\cite{Phongthawee2023DiffusionLight} & 6.76 & 0.26 & 0.20 \\
\toprule
\multirow{3}{*}{\shortstack[l]{Diffuse\\Sphere}} 
    & XiheNet~\cite{xihe_mobisys2021} & 11.8 & 0.12 & 0.21 \\
    & StyleLight~\cite{wang2022stylelight}        & 4.24 & 0.13 & 0.23 \\
    & DiffusionLight~\cite{Phongthawee2023DiffusionLight} & 2.14 & 0.14 & 0.20 \\
\midrule
\multirow{3}{*}{\shortstack[l]{Matte\\Sphere}} 
    & XiheNet~\cite{xihe_mobisys2021} & 12.2 & 0.17 & 0.23 \\
    & StyleLight~\cite{wang2022stylelight}        & 4.74 & 0.31 & 0.40 \\
    & DiffusionLight~\cite{Phongthawee2023DiffusionLight} & 3.42 & 0.33 & 0.36 \\
\midrule
\multirow{3}{*}{\shortstack[l]{Mirror\\Sphere}} 
    & XiheNet~\cite{xihe_mobisys2021} & 13.4 & 0.27 & 0.31 \\
    & StyleLight~\cite{wang2022stylelight}        & 6.78 & 0.55 & 0.51 \\
    & DiffusionLight~\cite{Phongthawee2023DiffusionLight} & 5.94 & 0.60 & 0.43 \\
\bottomrule
\end{tabular}

}
\vspace{-0.5cm}
\end{table}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% fig:case_study_lighting_result_visualizations
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{assets/lighting_estimation_case_study.pdf}
    \caption{Lighting estimation rendering visualizations. The \sysname visualization interface enables side-by-side display of virtual teapots under varying rendering parameters, such as different materials and lighting conditions. This design facilitates perceptual-based evaluation studies by supporting frame-by-frame visualization of numerical results from Table~\ref{tab:eval_three_sphere_reorganized}.
    }
\label{fig:case_study_lighting_result_visualizations}
\vspace{-0.5cm}
\end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{\sysname Setup}
\label{subsec:case_study_lighting_experimental_setup}

We evaluate three representative lighting estimation models, XiheNet~\cite{xihe_mobisys2021}, StyleLight~\cite{wang2022stylelight}, and DiffusionLight~\cite{Phongthawee2023DiffusionLight}. These models represent different tiers of estimation quality and model complexity. Specifically, XiheNet is a lightweight model that runs efficiently and generates low-frequency environment maps. StyleLight is a medium-sized model that offers improved visual quality. DiffusionLight, the largest among the three, produces the highest visual fidelity but with increased computational cost. These models run on \sysname as containerized programs. We conduct the evaluation using both numerical benchmarks and perceptual feedback on the rendered virtual objects. 
% \tian{briefly explain why they are representative, e.g., different lighting methods and outputs.}

For numerical evaluation, we first directly compared \emph{the estimated environment maps} using the Laval Indoor HDR testing dataset~\cite{Gardner2017}. We measure the estimation error using three commonly used evaluation metrics: angular error, scale-invariant root mean square error (Si-RMSE), and root mean square error, for the lighting estimation task~\cite{wang2022stylelight,Phongthawee2023DiffusionLight,somanath-envmapnet}. 

Additionally, we include numerical evaluation results using the \emph{three-sphere protocol}~\cite{wang2022stylelight}, which tests lighting estimation accuracy based on rendered objects instead of estimated environment maps. Three different object material types, diffuse, matte, and mirror, are included in this protocol to represent a wide range of common object material features. Fig.~\ref{fig:experiment_protocols} shows examples of the environment map and rendered virtual spheres as part of the numerical evaluation protocol. Setting up experiment protocols like the three-sphere protocol can be time-consuming and technically challenging for researchers and could cause adoption barriers. By supporting such standard evaluation protocols, \sysname allows easy-to-use and reproducible comprehensive evaluations of CV models.

For perceptual evaluation, we setup \sysname with the same edge-server configuration as described in \S\ref{sec:casestudy:depth}. The estimation model inputs were single-frame RGB captures with metadata streamed from an iPhone 14 Pro. All lighting estimation inferences were performed on the edge server using the built-in Three.js renderer. Rendering outputs, including rendered objects and environment maps, were saved and made accessible through our visualization interface. Specifically, as shown in Fig.~\ref{fig:case_study_lighting_result_visualizations}, the \sysname visualization interface enables side-by-side display of AR objects under varying rendering parameters, such as different object materials and lighting conditions.



\subsection{Interesting Findings}
% \subsection{Findings and Observations}
\label{subsec:case_study_lighting_findings_and_observations}

\para{Numerical Metric Discrepancies.}
Table~\ref{tab:eval_three_sphere_reorganized} shows quantitative results under the three-sphere protocol. Our evaluation reveals that different numerical metrics often highlight different aspects of lighting estimation performance. For instance, XiheNet achieves the lowest Si-RMSE in environment map-wise comparisons, yet it performs the worst in terms of angular error. This illustrates a key limitation of single-metric evaluation: while they provide convenient summaries, they are not expressive enough to capture the full spectrum of model behavior. And this is particularly true for visual realism. We suspect the reason is that metrics may emphasize different aspects, such as directional alignment or intensity differences, but none alone can fully account for how estimation errors manifest in rendered AR scenes. As a result, relying solely on these metrics can often lead to misleading or incorrect conclusions about a model’s true perceptual quality.


\begin{tcolorbox}[colback=gray!10, colframe=gray!50!black, boxrule=0.5pt, arc=2pt, left=4pt, right=4pt, top=2pt, bottom=2pt]
\textbf{Key Takeaway.} No single metric reliably captures all aspects of lighting estimation quality. \sysname makes it easy to observe that different metrics can yield conflicting conclusions. This finding also underscore the need for multi-metric evaluation and perceptual inspection, features provided by \sysname, especially when assessing visual realism in AR scenes.
\end{tcolorbox}


\para{Object Appearance and Spatial Context.} 
To better understand these numerical discrepancies, we use \sysname to visualize each model’s predictions under the same input conditions. As shown in Figure~\ref{fig:case_study_lighting_result_visualizations}, relit teapot rendered using different models reveal perceptual differences not captured in the numerical scores. While the quantitative metrics suggest that DiffusionLight performs best, visual inspection of the rendered objects uncovers nuanced issues, such as unnatural brightness or missing directional shadows. These issues would otherwise remain hidden in numerical-only evaluation. Thus, it is important to supplement numerical results with perceptual analysis when evaluating lighting estimation for AR.

We also observed that small inaccuracies in estimated light directions or intensities lead to large differences in object appearance, particularly in materials with specular components. For example, relighting with XiheNet resulted in over-smoothing of specular highlights, making the metallic teapot appear dull. By contrast, DiffusionLight sometimes overestimated intensity, causing teapots to look unnaturally bright under realistic indoor conditions. These artifacts are difficult to assess from environment maps alone, but become obvious when rendered into the AR scene using \sysname.
Such rendering results, generated using different configurations, can aid researchers in iteratively designing and conducting perception studies.

\begin{tcolorbox}[colback=gray!10, colframe=gray!50!black, boxrule=0.5pt, arc=2pt, left=4pt, right=4pt, top=2pt, bottom=2pt]
\textbf{Key Takeaway.} 
\sysname enables perceptual inspection of model outputs in consistent AR contexts, revealing artifacts---like missing shadows or unnatural brightness---that numerical metrics alone fail to capture. This capability is essential for evaluating lighting estimation models, where small prediction errors can cause large perceptual differences in object appearance, especially under specular materials.
\end{tcolorbox}

\subsection{Discussion and Implications}
\label{subsec:case_study_lighting_discussion_and_implications}

Our results confirm that existing lighting estimation metrics, though useful for benchmarking, are often insufficient to capture the perceptual quality of AR rendering fully. Even when two models achieve similar angular error or RMSE values, their outputs can diverge substantially in terms of user experience, especially when rendering more complex object materials. As AR systems demand increasingly realistic integration of virtual and physical elements, our case study provides good examples on using \sysname to evaluate models through numerical and perceptual methods.
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{assets/Architecture.pdf}
    \caption{System architecture of \sysname, illustrating its three main components and their associated modules.}
    \label{fig:architecture}
    \vspace{-0.5cm}
\end{figure}

